Capturing Conversion Rate Fluctuation during Sales Promotions: A Novel Historical Data Reuse Approach

Conversion rate (CVR) prediction is one of the core components in online recommender systems, and various approaches have been proposed to obtain accurate and well-calibrated CVR estimation. However, we observe that a well-trained CVR prediction model often performs sub-optimally during sales promotions. This can be largely ascribed to the problem of the data distribution shift, in which the conventional methods no longer work. To this end, we seek to develop alternative modeling techniques for CVR prediction. Observing similar purchase patterns across different promotions, we propose reusing the historical promotion data to capture the promotional conversion patterns. Herein, we propose a novel \textbf{H}istorical \textbf{D}ata \textbf{R}euse (\textbf{HDR}) approach that first retrieves historically similar promotion data and then fine-tunes the CVR prediction model with the acquired data for better adaptation to the promotion mode. HDR consists of three components: an automated data retrieval module that seeks similar data from historical promotions, a distribution shift correction module that re-weights the retrieved data for better aligning with the target promotion, and a TransBlock module that quickly fine-tunes the original model for better adaptation to the promotion mode. Experiments conducted with real-world data demonstrate the effectiveness of HDR, as it improves both ranking and calibration metrics to a large extent. HDR has also been deployed on the display advertising system in Alibaba, bringing a lift of $9\%$ RPM and $16\%$ CVR during Double 11 Sales in 2022.

==> chapters/drop-2-preliminaries.tex <==
\section{Preliminaries} 
\label{sec:prelim}
% \subsection{Problem Formulation} 


% \subsection{Delayed Feedback in CVR} 
% Unlike click behavior whose feedback happens timely, the user conversion action may occur hours or days later. Therefore, the conversion distribution is closely dependent on the observation time which is called the attribution window. For example, a user clicks on an item and buys the one the next day. In the first case, the attribution window is set to 1 day, this click does not introduce a conversion within this day, so this record is a negative sample in the data at this time. When the attribution window is stretched to 2 days, this record is converted to a positive sample because a purchase occurs on the second day. In practice, industrial systems often set the length of the attribution window according to their own business needs, that is, it estimates the CVR during this period after click. For example, the Alibaba advertisement platform often estimates the CVR during 3 days after the click action happened i.e., the attribution window is 3 days. Therefore, the unambiguous distribution of conversion labels of T day is not available until ending of T+2 days. 

% Industrial recommender systems usually refresh their prediction models on recent data in a timely manner to capture real-time user behavior. Waiting until the end of the attribution window can cause the data obsolete which makes the model's performance sub-optimal. In practice, it often set a waiting window whose length is suitable to refresh the CVR prediction model via recent real-time data. Herein, all samples that exceed the waiting window are considered negative samples, except for those undergoing conversion in the waiting window. Those data are representative of the observed distribution $p(x,y')$. There are some conversions that happened beyond the waiting window but within the attribution window. Thus, the negative samples in the observed distribution are biased. Recent studies often utilize weighted sampling to correct the distribution bias. We indicate the actual distribution as $p(x,y)$, 
% \begin{equation}
% \begin{aligned}
% p(x,y) = w(x, y, y') \cdot p(x,y')
% \end{aligned}
% \end{equation}
% where $w(x, y, y')$ is often derived based on the relationship between the recently observed distribution and actual distribution, and recent works often design neural networks to infer it. For example, we can obtain the data with the labels of conversion in one day (called CVR1d) when the day ends if we set the waiting window to 1 day. Besides, we count that CVR1d/CVR3d is generally 81\%, thus we calibrate the bias between the observed and actual distributions by $w(x, y, y')$ calculated by CVR1d/CVR3d. In general, the stability of the gap between the observed and actual distributions affects the effectiveness of $w(x, y, y')$. For example, we obtain the data with the labels of conversion in one day (called CVR1d) when the day ends if we set the waiting window to 1 day. Besides, we count that CVR1d/CVR3d is generally 81\%, thus we calibrate the bias between the observed and actual distributions by $w(x, y, y')$ calculated by CVR1d/CVR3d. If the ratio changes significantly, weighted sampling can only perform sub-optimal. 

% \begin{table}[]
% \caption{We use the CVR under 1-day or 2-day waiting window, i.e., CVR1d and CVR2d, epochs to indicate the gap between the observed and actual distributions, i.e., CVR3d. 2022/05/29 is the second day before the Double 11 Sale, and 2022/11/03 is the last day of the day when the discount prices take effect.}
% \centering
% \begin{tabular}{ccc}
% \toprule
% Date & CVR1d/CVR3d & CVR2d/CVR3d \\ \midrule
% Daily & 81.6\% & 93.5\% \\ 
% 2022/10/29 & 28.3\% & 48.6\% \\ 
% 2022/11/03 & 89.2\% & 97.8\% \\ 
% \bottomrule
% \end{tabular}
% % \begin{tablenotes}%[para,flushleft]
% % \item[a] xxx
% % \end{tablenotes}
% \label{table:yy_gap}
% \end{table} 

% \subsection{Why CVR Estimation Suffers from Sales Promotions?} 
% The online recommendation systems work based on the i.i.d assumption that the history distribution used for model training and the inferred real-time distribution are independent identical distributions. However, the i.i.d assumption obviously can not hold in the sales promotions, that is user behavior during the promotion cycle is quite different from daily. For example, cosmetics often have high price tags daily, however, the discounted price in promotions is often significantly lower than the daily price. As a result, there is a significant increase in the CVR of cosmetics in promotions. In general, the prediction model needs real-time data that can represent the promotion distribution to fine-tune the parameters to handle the distribution shift. 

% However, the real-time data in the promotion, i.e. the observed distribution, has a huge gap from the actual distribution. We take Taobao Double 11 Sales for example. During the two days before the discount price takes effect, most clicks do not have a corresponding conversion tag until the discount day arrives, because people often would like to obtain things at the lower discount price. However, when the discount price takes effect, those clicks will become positive conversion samples rapidly. As shown in Table~\ref{table:yy_gap}, the CVR1d/CVR3d in 2022/05/29, i.e., the second day before the Double 11 Sale, is 28.3\% which is much lower than the common daily 81.6\%. As mentioned above, the recent delayed feedback modeling approach fails when the gap between the observed and the actual distribution changes significantly. Therefore, recent CVR estimation methods, with or without delayed feedback modeling, are not able to predict CVR under such distribution saltation in sales promotions. 


% \subsection{Problem Formulation} 
% Towards clear statements, we first formulate the CVR estimation during sales promotion. We use $f_\Theta$ to indicate the CVR prediction model, where $\Theta$ is the trainable parameters. The distribution of the training data is denoted by $\mathcal{D}(x, y)$, while the actual data distribution in the inference procedure, i.e., the target distribution, is $p(x,y)$. 
% In general, the online recommendation systems work based on the i.i.d assumption that the training distribution $\mathcal{D}(x, y)$ and the inferred real-time distribution $p(x,y)$ are independent identical distributions. However, the i.i.d assumption obviously can not hold in the sales promotions, that is user behavior during the promotion cycle is quite different from daily. For example, cosmetics often have high price tags daily, however, the discounted price in promotions is often significantly lower than the daily price. As a result, there is a significant increase in the CVR of cosmetics in sales promotion. Therefore, we shall let the CVR prediction model adapt to the target distribution $p(x,y)$ which is non-accessible. 

% \subsection{Why CVR Estimation Suffers from Sales Promotions?} 

% \begin{table}[]
% \caption{We use the CVR under 1-day or 2-day waiting window, i.e., CVR1d and CVR2d, epochs to indicate the gap between the observed and actual distributions, i.e., CVR3d. 2022/05/29 is the second day before the Double 11 Sale, and 2022/11/03 is the last day of the day when the discount prices take effect.}
% \centering
% \begin{tabular}{ccc}
% \toprule
% Date & CVR1d/CVR3d & CVR2d/CVR3d \\ \midrule
% Daily & 81.6\% & 93.5\% \\ 
% 2022/10/29 & 28.3\% & 48.6\% \\ 
% 2022/11/03 & 89.2\% & 97.8\% \\ 
% \bottomrule
% \end{tabular}
% \label{table:yy_gap}
% \end{table} 

% As mentioned above,  the i.i.d assumption can not hold in the sales promotions because the conversion distribution in promo shifts. Therefore, the performance of the CVR estimation degrades significantly if there is no countermeasure to handle this shifting issue. Industrial recommender systems often handle refresh their prediction models on recent data in a timely manner to handle such a shifting issue. However, the utilization of recent data in CVR estimation needs to consider the delayed feedback problem. 

% Unlike click behavior whose feedback happens timely, the user conversion action may occur hours or days later. In practice, industrial systems often set the length of the attribution window according to their own business needs, that is, it estimates the CVR during this period after click. For example, the Alibaba advertisement platform often estimates the CVR during 3 natural days after the click action happened i.e., the attribution window is 3 days. Therefore, the unambiguous distribution of conversion labels of T day is not available until ending of T+2 days. 

% Waiting until the end of the attribution window can cause the data obsolete which makes the model's performance sub-optimal. In practice, it often set a waiting window whose length is suitable to refresh the CVR prediction model via recent real-time data. Herein, all samples that exceed the waiting window are considered negative samples, except for those undergoing conversion in the waiting window. Those data are representative of the observed distribution $p(x,y')$. There are some conversions that happened beyond the waiting window but within the attribution window. Thus, the negative samples in the observed distribution are biased. Recent studies often utilize weighted sampling to correct the distribution bias. We indicate the actual distribution as $p(x,y)$, 
% \begin{equation}
% \begin{aligned}
% p(x,y) = w(x, y, y') \cdot p(x,y')
% \end{aligned}
% \end{equation}
% where $w(x, y, y')$ is often derived based on the relationship between the recently observed distribution and actual distribution, and recent works often design neural networks to infer it. In general, the stability of the gap between the observed and actual distributions affects the effectiveness of $w(x, y, y')$. For example, we obtain the data with the labels of conversion in one day (called CVR1d) when the day ends if we set the waiting window to 1 day. Besides, we count that CVR1d/CVR3d is generally 81\%, thus we calibrate the bias between the observed and actual distributions by $w(x, y, y')$ calculated by CVR1d/CVR3d. If the ratio changes significantly, the delayed feedback modeling can only perform sub-optimally. 
% \chan{In this work, we attempt to hold on breakthrough point by reusing historical promotion data.}

% \subsection{Overfitting in Recommender System}
% Since we consider reusing historical data, we need to face a problem specific to deep learning of recommender systems, i.e., one-epoch phenomenon. Different from overfitting in tasks like computer vision, where the model is usually trained for tens even hundreds of epochs, and the overfitting occurs gradually. In recommender system, it is that model performance increases gradually within the first epoch while falls dramatically at the beginning of the second epoch. This phenomenon is referred to as the one-epoch phenomenon. \chan{Zhang et al.} summerize the overfitting phenomenon of the deep user behavior prediction model and conclude it as the embeddngs becomes discriminatory upon positive and negative samples after the first epoch training. It make the MLP can  distinguish positive and negative samples easily, and thus optimization of model could obtain easily a trivial solution which is not generalizable. 

% In practical industrial systems, recommendation model often load well-trained parameters from the last version and consume the latest data samples, which leads better performance. Such a training process may continue for a long period of time, even for years, in industrial systems like the displaying advertisement system of Alibaba. Due to historical data has been used for model training, it means that we need to solve the overfitting caused by the one-epoch phenomenon when we conduct data reuse. 


\section{Problem Formulation} 
\label{sec:prelim} 

%\subsection{Problem Formulation} 
%We firstly formulate the CVR estimation during sales promotion. We use $f_\Theta$ to indicate the CVR prediction model, where $\Theta$ is the trainable parameters. The distribution of the training data is denoted by $\mathcal{A}(x, y)$, while the actual data distribution in the inference procedure, i.e., the target distribution, is $\mathcal{B}(x, y)$. 
%In general, the online recommendation systems work based on the i.i.d assumption that the training distribution $\mathcal{A}(x, y)$ and the inferred real-time distribution $\mathcal{B}(x, y)$ are independent identical distributions. However, the i.i.d assumption obviously can not hold in the sales promotions, that is user behavior during the promotion cycle is quite different from daily. For example, cosmetics often have high price tags daily, however, the discounted price in promotions is often significantly lower than the daily price. As a result, there is a significant increase in the CVR of cosmetics in sales promotion. Therefore, we shall let the CVR prediction model adapt to the target distribution $\mathcal{B}(x, y)$ which is non-accessible. 

\begin{table}[]
\caption{We use the CVR under 1-day or 2-day waiting window, i.e., CVR1d and CVR2d, epochs to indicate the gap between the observed and actual distributions, i.e., CVR3d. 2022/05/29 is the second day before the Double 11 Sale, and 2022/11/03 is the last day of the day when the discount prices take effect.}
\centering
\begin{tabular}{ccc}
\toprule
Date & CVR1d/CVR3d & CVR2d/CVR3d \\ \midrule
Daily & 81.6\% & 93.5\% \\ 
2022/10/29 & 28.3\% & 48.6\% \\ 
2022/11/03 & 89.2\% & 97.8\% \\ 
\bottomrule
\end{tabular}
% \begin{tablenotes}%[para,flushleft]
% \item[a] xxx
% \end{tablenotes}
\label{table:yy_gap}
\end{table} 

We firstly formulate the CVR estimation degeneration problem during sales promotion. We denote $f_\Theta$ to indicate the CVR prediction model, where the model is well-trained in an online learning manner and $\Theta$ is trainable parameters. The distribution of the recent training data is represented as $\mathcal{A}(x, y)$, while the actual online distribution in the inference procedure, i.e., the inference/target distribution, is $\mathcal{B}(x, y)$. Note that the complete $\mathcal{B}(x, y)$ is unobservable during model training. The online recommendation systems work based on the i.i.d assumption, i.e., it requires that the training distribution $\mathcal{A}(x, y)$ and the inference distribution $\mathcal{B}(x, y)$ are independent identical distributions. 

We summarize the essential cause of the CVR estimation degeneration problem during sales promotion is that the difference between training distribution $\mathcal{A}(x, y)$ and inference distribution $\mathcal{B}(x, y)$ is so large that the i.i.d assumption could not hold during the sales promotion. This problem comes from user behavior during the promotion cycle is quite different from daily. For example, cosmetics often have high price tags daily, however, the discounted price in promotion is often significantly lower. As a result, users are more likely to buy cosmetics during promotion than on a daily basis. It causes a significant increase in the CVR of cosmetics in sales promotion. Therefore, the performance of the CVR prediction model degrades significantly if there is no countermeasure to handle this distribution shifting issue. 

Industrial recommender systems often handle refresh their prediction models on recent data in a timely manner to handle such a shifting issue. However, the utilization of recent data in CVR estimation needs to consider the delayed feedback problem. Unlike click behavior whose feedback happens timely, the user conversion action may occur hours or days later. In practice, industrial systems often set the length of the attribution window according to their own business needs, that is, it estimates the CVR during this period after click\footnote{For example, the Alibaba advertisement platform often estimates the CVR during 3 natural days after the click action happened i.e., the attribution window is 3 days. Therefore, the unambiguous distribution of conversion labels of T day is not available until ending of T+2 days.}.

Waiting until the end of the attribution window can cause the data obsolete which makes the model's performance sub-optimal. In practice, it often set a waiting window whose length is suitable to refresh the CVR prediction model via recent real-time data. Herein, all samples that exceed the waiting window are considered negative samples, except for those undergoing conversion in the waiting window. Those data are representative of the observed distribution $p(x,y')$. There are some conversions that happened beyond the waiting window but within the attribution window. Thus, the negative samples in the observed distribution are biased. Recent studies often utilize weighted sampling to correct the distribution bias. We indicate the actual distribution as $p(x,y)$, 
\begin{equation}
\begin{aligned}
p(x,y) = w(x, y, y') \cdot p(x,y')
\end{aligned}
\end{equation}
where $w(x, y, y')$ is often derived based on the relationship between the recently observed distribution and actual distribution, and recent works often design neural networks to infer it. In general, the stability of the gap between the observed and actual distributions affects the effectiveness of $w(x, y, y')$. For example, we obtain the data with the labels of conversion in one day (called CVR1d) when the day ends if we set the waiting window to 1 day. Besides, we count that CVR1d/CVR3d is generally 81\%, thus we calibrate the bias between the observed and actual distributions by $w(x, y, y')$ calculated by CVR1d/CVR3d. If the ratio changes significantly, the delayed feedback modeling can only perform sub-optimally. 

In this work, we attempt to reuse historical promotion data to handle such sub-optimal performance. 

\section{Preliminaries} 
\subsection{Importance-Weighted Empirical Risk Minimization} 
Empirical risk minimization (ERM) is a principle in statistical learning theory which is the basis of many classical machine learning algorithms, e.g., supervised learning. The core idea is that we cannot know exactly how well an algorithm will work in practice (the true "risk") because we don't know the true distribution of data that the algorithm will work on, but we can instead measure its performance on a known set of training data $q(x,y)$ as 
\begin{equation}
\begin{aligned}
\label{eq:erm} 
%\mathcal{L} &= \sum_{(x,y) \in q(x,y)}\ell(x,y), 
\mathcal{L} &= \int \ell(x,y) \ \mathrm{d} q(x,y) 
\end{aligned}
\end{equation}
where $\ell$ indicates the loss function, e.g., cross-entropy loss and mean squared error. However, In practice, the distribution of the training data could differ from the target/inference distribution which is called distribution shift. \chan{Shimodaira}~\footnote{\chan{Paper: Improving predictive inference under covariate shift by weighting the log-likelihood function}} proposed Importance-Weighted ERM to handle such distribution shift as 
\begin{equation}
\begin{aligned}
\label{eq:iw_erm} 
%\mathcal{L} &= \frac{p(x,y)}{q(x,y)} \cdot \ell_{(x,y) \in q(x,y)}(x,y), 
\mathcal{L} &= \int \frac{p(x,y)}{q(x,y)} \cdot \ell(x,y) \ \mathrm{d} q(x,y) 
\end{aligned}
\end{equation}
where $p(x,y)$ and $q(x,y)$ indicate training distribution and target/inference distribution. Importance-Weighted ERM is the theoretical basis for many domain adaptation methods.~\chan{TODO: cite} 


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.9\columnwidth]{figs/odl.pdf} 
%     \caption{An illustration of the online learning process for industrial recommender systems.} 
%     \label{fig:odl}
% \end{figure}


\subsection{Overfitting in Recommender System}
Since we consider reusing historical data, we need to face a problem specific to deep learning of recommender systems, i.e., one-epoch phenomenon. Different from overfitting in tasks like computer vision, where the model is usually trained for tens even hundreds of epochs, and the overfitting occurs gradually. In recommender system, it is that model performance increases gradually within the first epoch while falls dramatically at the beginning of the second epoch. This phenomenon is referred to as the one-epoch phenomenon. \chan{Zhang et al.} summerize the overfitting phenomenon of the deep user behavior prediction model and conclude it as the embeddngs becomes discriminatory upon positive and negative samples after the first epoch training. It make the MLP can  distinguish positive and negative samples easily, and thus optimization of model could obtain easily a trivial solution which is not generalizable. 

In practical industrial systems, recommendation model often load well-trained parameters from the last version and consume the latest data samples, which leads better performance. Such a training process may continue for a long period of time, even for years, in industrial systems like the displaying advertisement system of Alibaba. Due to historical data has been used for model training, it means that we need to solve the overfitting caused by the one-epoch phenomenon when we conduct data reuse. 


%\subsection{Why CVR Estimation Suffers from Sales Promotions?} 


%\subsection{Delay Feedback in CVR} 
%Unlike click behavior whose feedback happens timely, the user conversion action may occur hours or days later. Therefore, the conversion distribution is closely dependent on the observation time which is called the attribution window. For example, a user clicks on an item and buys the one the next day. In the first case, the attribution window is set to 1 day, this click does not introduce a conversion within this day, so this record is a negative sample in the data at this time. When the attribution window is stretched to 2 days, this record is converted to a positive sample because a purchase occurs on the second day. In practice, industrial systems often set the length of the attribution window according to their own business needs, that is, it estimates the CVR during this period after click. For example, the Alibaba advertisement platform often estimates the CVR during 3 days after the click action happened i.e., the attribution window is 3 days. Therefore, the unambiguous distribution of conversion labels of T day is not available until ending of T+2 days. 

%Industrial recommender systems usually refresh their prediction models on recent data in a timely manner to capture real-time user behavior. Waiting until the end of the attribution window can cause the data obsolete which makes the model's performance sub-optimal. In practice, it often set a waiting window whose length is suitable to refresh the CVR prediction model via recent real-time data. Herein, all samples that exceed the waiting window are considered negative samples, except for those undergoing conversion in the waiting window. Those data are representative of the observed distribution $p(x,y')$. There are some conversions that happened beyond the waiting window but within the attribution window. Thus, the negative samples in the observed distribution are biased. Recent studies often utilize weighted sampling to correct the distribution bias. We indicate the actual distribution as $p(x,y)$, 
%\begin{equation}
%\begin{aligned}
%p(x,y) = w(x, y, y') \cdot p(x,y')
%\end{aligned}
%\end{equation}
%where $w(x, y, y')$ is often derived based on the relationship between the recently observed distribution and actual distribution, and recent works often design neural networks to infer it. For example, we can obtain the data with the labels of conversion in one day (called CVR1d) when the day ends if we set the waiting window to 1 day. Besides, we count that CVR1d/CVR3d is generally 81\%, thus we calibrate the bias between the observed and actual distributions by $w(x, y, y')$ calculated by CVR1d/CVR3d. In general, the stability of the gap between the observed and actual distributions affects the effectiveness of $w(x, y, y')$. For example, we obtain the data with the labels of conversion in one day (called CVR1d) when the day ends if we set the waiting window to 1 day. Besides, we count that CVR1d/CVR3d is generally 81\%, thus we calibrate the bias between the observed and actual distributions by $w(x, y, y')$ calculated by CVR1d/CVR3d. If the ratio changes significantly, weighted sampling can only perform sub-optimal. 

%As mentioned above,  the i.i.d assumption can not hold in the sales promotions because the conversion distribution in promo shifts. Therefore, the performance of the CVR estimation degrades significantly if there is no countermeasure to handle this shifting issue. Industrial recommender systems often handle refresh their prediction models on recent data in a timely manner to handle such a shifting issue. However, the utilization of recent data in CVR estimation needs to consider the delayed feedback problem. 
%
%Unlike click behavior whose feedback happens timely, the user conversion action may occur hours or days later. In practice, industrial systems often set the length of the attribution window according to their own business needs, that is, it estimates the CVR during this period after click. For example, the Alibaba advertisement platform often estimates the CVR during 3 natural days after the click action happened i.e., the attribution window is 3 days. Therefore, the unambiguous distribution of conversion labels of T day is not available until ending of T+2 days. 
%
%Waiting until the end of the attribution window can cause the data obsolete which makes the model's performance sub-optimal. In practice, it often set a waiting window whose length is suitable to refresh the CVR prediction model via recent real-time data. Herein, all samples that exceed the waiting window are considered negative samples, except for those undergoing conversion in the waiting window. Those data are representative of the observed distribution $p(x,y')$. There are some conversions that happened beyond the waiting window but within the attribution window. Thus, the negative samples in the observed distribution are biased. Recent studies often utilize weighted sampling to correct the distribution bias. We indicate the actual distribution as $p(x,y)$, 
%\begin{equation}
%\begin{aligned}
%p(x,y) = w(x, y, y') \cdot p(x,y')
%\end{aligned}
%\end{equation}
%where $w(x, y, y')$ is often derived based on the relationship between the recently observed distribution and actual distribution, and recent works often design neural networks to infer it. In general, the stability of the gap between the observed and actual distributions affects the effectiveness of $w(x, y, y')$. For example, we obtain the data with the labels of conversion in one day (called CVR1d) when the day ends if we set the waiting window to 1 day. Besides, we count that CVR1d/CVR3d is generally 81\%, thus we calibrate the bias between the observed and actual distributions by $w(x, y, y')$ calculated by CVR1d/CVR3d. If the ratio changes significantly, the delayed feedback modeling can only perform sub-optimally. 
%\chan{In this work, we attempt to hold on breakthrough point by reusing historical promotion data.}


%\subsection{Why CVR Estimation Suffers from Sales Promotions?} 
%The online recommendation systems work based on the i.i.d assumption that the history distribution used for model training and the inferred real-time distribution are independent identical distributions. However, the i.i.d assumption obviously can not hold in the sales promotions, that is user behavior during the promotion cycle is quite different from daily. For example, cosmetics often have high price tags daily, however, the discounted price in promotions is often significantly lower than the daily price. As a result, there is a significant increase in the CVR of cosmetics in promotions. In general, the prediction model needs real-time data that can represent the promotion distribution to fine-tune the parameters to handle the distribution shift. 
%
%However, the real-time data in the promotion, i.e. the observed distribution, has a huge gap from the actual distribution. We take Taobao Double 11 Sales for example. During the two days before the discount price takes effect, most clicks do not have a corresponding conversion tag until the discount day arrives, because people often would like to obtain things at the lower discount price. However, when the discount price takes effect, those clicks will become positive conversion samples rapidly. As shown in Table~\ref{table:yy_gap}, the CVR1d/CVR3d in 2022/05/29, i.e., the second day before the Double 11 Sale, is 28.3\% which is much lower than the common daily 81.6\%. As mentioned above, the recent delayed feedback modeling approach fails when the gap between the observed and the actual distribution changes significantly. Therefore, recent CVR estimation methods, with or without delayed feedback modeling, are not able to predict CVR under such distribution saltation in sales promotions. 



==> chapters/drop-3-model-bak.tex <==
% \section{The Proposed Method} 
% \label{sec:model} 

% \subsection{Observation and Motivation} 
% As mentioned before, recent CVR estimation methods, with or without delayed feedback modeling, are not able to predict CVR under such distribution saltation in sales promotions. To this end, we explore CVR estimation in sales promotions from a novel idea. 

% First of all, through observing the trend of CVR, we find that the CVR between the sales promotions is closer than the promotions' and daily's. Thus, the intuitive idea is whether we could utilize the data of historical promotions to make the CVR model adapt to distribution during promotion. Thereafter, we analyze the statistics among the sales promotions and are aware of that the distribution of similar promotion approximately conform to the label shift assumption. Specifically, we indicate the distribution of promotion A and B by $\mathcal{A}(x, y)$ and $\mathcal{B}(x,y)$, respectively, we can obtain $\mathcal{A}(x|y)=\mathcal{B}(x|y)$. 
% The intuitive understanding is that similar groups of users often select similar products in two similar promotions. To support this assumption, we counted the relevant data and verified its reasonable. \chan{TODO: data} 

% Therefore, we propose a novel idea of CVR estimation: treating CVR estimation as a distribution adaptation problem under the \textit{label shift} assumption. Specifically, we propose the following two-stage algorithmic framework. Firstly, we design an efficient retrieval approach to search the historical data close to the current distribution in terms of day-level data. 
% Secondly, we propose a distribution adaptation algorithm based on the importance-weighted Empirical Risk Minimization (ERM) framework, which can adapt the CVR model to the current target distribution based on the retrieved historical data and a fraction of real-time data without conversion label. Note that we find that the model perform overfitting while fine-tuning the model with historical data, that is the one-epoch phenomenon in recommendation system. Therefore, we designed a plug-and-play TransBlock module to alleviate the overfitting problem. 

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{figs/vector_index_building.jpg} 
%     \caption{The overall of the vector index building.} 
% \end{figure} 

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{figs/pre_index.jpg} 
%     \caption{The overall of TransBlock.} 
% \end{figure} 

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{figs/p_x_given_y.jpg} 
%     \caption{The overall of TransBlock.} 
% \end{figure} 


% \subsection{Vector-Based Retrieval} 
% %Firstly, we design an efficient retrieval approach to search the historical data close to the current distribution in terms of day-level data.
% In the first step of the algorithm flow, we seek to obtain historical data that is similar with real-time distribution and approximately conform the label shift assumption. To industrial production deployment, we should avoid manual selection, and thus we build a vector-based retrieval approach in non-parametric manner to automatically retrieval similar data. In this following work, we set the retrieval granularity into day-level data, that is we shall select one day in historical data, whose data distribution is close to the current day's. 

% \subsubsection{Vector-based index building} 
% \label{sec:index_building}
% Due to the lack of data for training, we do not follow the data-driven manner, and return to classical feature engineering. Specifically, we analyzed observable data during the promotion and mined the feature factors that can represent to the characteristic of data distribution. 

% First, we do not have access to the full target distribution, because our target is the current day-level data distribution $p(x,y)$, where $p(x)$ is available at the end of the day, and the waiting time for $p(y)$ is even as long as the attribution window. To this end, we explore the CVR trend during the promotion: the real-time conversion decreases significantly in the period before the discounted price takes effect, increases significantly when the discounted price takes effect, and decreases significantly again after the termination of the promotion. Therefore, we proposed to utilize the statistic from several preceding days to represent the unavailable current day. 
% Meanwhile, we analyze the observable data. As shown in figure 2, we are aware that the trend of the display ratio of some specific categories is similar to the trend of CVR during the promotion. Therefore, we selected the display ratio of several representative categories as the feature factors for the retrieval. 

% Specifically, we select seven representative product categories and count their display ratios in three preceding days of the current day. 
% In the experiments, we find that if we consider statistics from the current day, it could significantly improve the performance of retrieval. Under the consideration of the retrieval effectiveness and the delay of the model serving, we also count the selected categories' display ratio of the first 10 hours of the current day. 
% Thereafter, we build 28-dimensional vectors which are utilized as the retrieval indexes for the current day. 


% \subsubsection{Retrieval method} 
% Based on the constructed vector-based index, we design a simple and efficient non-parametric vector retrieval methods. We calculate the cosine distance between the index of current day $\text{T}_\text{target}$ and the historical day $\text{T}_\text{history}$ as the similarity score: 
% \begin{equation}
% \begin{aligned}
% \label{eq:retieval} 
% S_\text{similar} = \frac{V_\text{target} \cdot V_\text{history}}{|V_\text{target}| \cdot |V_\text{history}|} 
% \end{aligned}
% \end{equation}
% Finally, we select the historical data with Top-3 similarity as the search result, so as to retrieve the most similar historical data.

% \subsection{CVR Estimation} 
% After obtaining the available similar historical data through the above retrieval procedure, we conduct the estimation for accurate CVR with retrieved historical data and predictive score during the first 10 hours of the current day. Inspired by Black Box Shift Estimation (BBSE) approach for domain adaptation under label shift assumption, we regard the CVR estimation task as a domain adaptation task under label shift assumption, where the source domain is historical data. 

% After obtaining the available similar historical data through the above retrieval procedure, we conduct the estimation for accurate CVR with retrieved historical data and predictive score during the first 10 hours of the current day. Inspired by Black Box Shift Estimation (BBSE) approach under label shift assumption, we design the CVR estimation under the importance-weighted ERM framework. The framework fine-tunes the current CVR prediction model on the following loss function, 
% \begin{equation}
% \begin{aligned}
% \label{eq:retieval} 
% \mathcal{L} &= \frac{p(x,y)}{q(x,y)} \cdot \ell_{(x,y) \in q(x,y)}(x,y) \\ 
% &= \frac{p(x|y) \cdot p(y)}{q(x|y) \cdot q(y)} \cdot \ell_{(x,y) \in q(x,y)}(x,y) \\
% %&= \frac{\overbrace{p(y)}^{unknown}}{\underbrace{q(y)}_{accessible}} \cdot \ell_{(x,y) \in q(x,y)}(x,y), 
% &= \frac{p(y)}{q(y)} \cdot \ell_{(x,y) \in q(x,y)}(x,y), 
% \end{aligned}
% \end{equation}
% where $\ell$ is the loss function and it is cross-entropy in this work. $p(x,y)$ and $q(x,y)$ indicate the target distribution and historical distribution, respectively. As mentioned above, we assume the historical distribution and target distribution conform the \textit{label shift} setting, i.e., $p(x|y)=q(x|y)$. 

% Since q(y) is known, we need to obtain the target label distribution p(y). However, it's hard to work out p(y), thus we change the target. As shown in Figure 1, the CVR ratio at any corresponding time between two days is relatively stable. We replace the $\frac{p(y)}{q(y)}$ by the ratio between the part of the day, as following, 
% \begin{equation}
% \begin{aligned}
% \label{eq:retieval} 
% \frac{p(y)}{q(y)} &\approx \frac{p^{h}(y)}{q^{h}(y)}, 
% \end{aligned} 
% \end{equation}
% where $q^{h}(y)$ is also available, thereafter, we seek to solve the $p^h(y)$. 

% Denote by $\hat{y} = f(x)$ the output of a fixed function $f$ which is a trained classifier, we arrive that $p^h(\hat{y}|y)=q^h(\hat{y}|y)$ when $p^h(x|y)=q^h(x|y)$ holds. %: $\mathcal{X} \rightarrow \mathcal{Y}$. 
% Hereafter, we combine the law of total probability and arrive at
% \begin{equation}
% \begin{aligned}
% \label{eq:s} 
% p^h(\hat{y}) 
% &= \int p^h(\hat{y}|y) \cdot p^h(y) \ \mathrm{d}y \\
% &= \int q^h(\hat{y}|y) \cdot p^h(y) \ \mathrm{d}y, 
% %&= \sum_{y \in (0,1)} p^h(\hat{y}|y) \cdot p^h(y) \\ 
% %&= \sum_{y \in (0,1)} q^h(\hat{y}|y) \cdot p^h(y), 
% \end{aligned} 
% \end{equation} 
% where we can obtain $p^h(\hat{y})$ and $q^h(\hat{y})$ through using classifier $f$ to score the $p^h(x)$ and $q^h(x)$. Due to the historical data being fully labeled, we can obtain $q^h(\hat{y}|y)$ from $q^h(\hat{y})$ according to the labels. For the convenience of representation, we write the above formula in matrix form as 

% \begin{equation}
% \begin{aligned}
% \label{eq:matrix} 
% %\hat{s} &= 
% %\begin{pmatrix}  
% %  \hat{s}_{y=1} & \hat{s}_{y=0} 
% %\end{pmatrix} \cdot 
% %\begin{pmatrix}  
% %  s_{y=1} \\ 
% %  s_{y=0} 
% %\end{pmatrix} \\ 
% D(\hat{y}) &= D(\hat{y}|y) \cdot D(y). 
% \end{aligned} 
% \end{equation} 
% To solve $D(y)$, we can construct the following problem as 

% \begin{equation}
% \begin{aligned}
% \label{eq:problem} 
% \mathop{\arg\min}_{D(y)} \underbrace{|| D(\hat{y}|y) \cdot D(y) - D(\hat{y}) ||^2}_\text{(a)} + \underbrace{\lambda \cdot || D(\hat{y}) - D(y) ||^2 }_\text{(b)} 
% \end{aligned} 
% \end{equation} 
% where Eq.(a) is to solve the Eq.~\ref{eq:matrix}, and Eq.(b) is a regularization constraint that constrains $\frac{p(y)}{q(y)}$ close to 1 for stability during training. \chan{cite} By solving Eq.~\ref{eq:problem}, we can obtain a closed-form solution $p^h(y)$ as
% \begin{equation}
% \begin{aligned}
% \label{eq:y} 
% D(y) = (D(\hat{y}|y)^TD(\hat{y}|y) + \lambda \mathbf{I})^{-1}(D(\hat{y}|y)^TD(\hat{y}) + \lambda D(y'). 
% \end{aligned} 
% \end{equation} 
% Thus, we work out the $\frac{p^h(y)}{q^h(y)}$. Finally, we could fine-tune CVR prediction model according to \chan{Eq. 3} to adopt the promotion. 

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{figs/transblock.jpg} 
%     \caption{The overall of TransBlock.} 
% \end{figure} 

% \subsection{Tuning based on TransBlock Module} 
% Due to the one-epoch phenomenon in recommender system, there will be terrible overfitting in fine-tuning procedure. Thus, we design a plug-and-play TransBlock module to assist fine-tuning and avoid the overfitting from historical data reusing. TransBlock is a stacking layer that is independent of the CVR model structure, and its goal is residuals of original predictive CVR score to ideal value.

% \subsubsection{Motivation}  We use stacked design to protect the original predictive ability of the CVR model by optimizing the added stacking parameters more and original model less through historical data. Due to the sparsity of retrieved day-level historical data, we could only add a small amount of parameters to ensure convergence on the limited data. Thus, we design TransBlock as following intuitive considering, 
% \begin{equation}
% \begin{aligned}
% \label{eq:transblock} 
% p_\text{ideal}(y=1|x) = p(y=1|x) + \underbrace{v_{(x)} \cdot p(y=0|x)}_\text{(a)} - \underbrace{u_{(x)} \cdot p(y=1|x)}_\text{(b)}
% \end{aligned} 
% \end{equation} 
% where the $p(y=1|x)$ and $p(y=0|x)$ are the conversion rate and non-conversion rate calculated by original CVR prediction model. The parts of above equation are 
% \begin{itemize}%[leftmargin=*]
% \item (a). \textit{Predicted probability of non-conversion but conversion, e.g., some products are rarely purchased on a daily basis, but are purchased frequently during sales promotion;} 
% \item (b). \textit{Predicted probability of conversion but non-conversion, e.g., some products that are frequently purchased on a daily basis, but rarely during sales promotion,} 
% \end{itemize} 
% where $u_{(x)}$ and $v_{(x)}$ are the sample-related transfer probabilities. We further simplify the formula and arrive the calculation process of TransBlock, 
% \begin{equation}
% \begin{aligned}
% \label{eq:transblock} 
% p_\text{trans}(y=1|x) 
% =& p(y=1|x) + v_{(x)} \cdot p(y=0|x) - u_{(x)} \cdot p(y=1|x) \\ 
% =& p(y=1|x) + v_{(x)} \cdot p(y=0|x) - u_{(x)} \cdot (1-p(y=0|x)) \\
% =& p(y=1|x) + (v_{(x)}+u_{(x)}) \cdot p(y=0|x) - u_{(x)} \\
% \rightarrow & p(y=1|x) + \underbrace{w_{(x)} \cdot p(y=0|x) + b_{(x)}}_{w_{(x)}=v_{(x)}+u_{(x)}, b_{(x)}=-u_{(x)}}. 
% %\small{\text{where} \ w_{(x)}=v_{(x)}+u_{(x)}, b_{(x)}=-u_{(x)}}
% \end{aligned} 
% \end{equation} 
% As mentioned above, the TransBlock module takes the non-conversion probability $p(y=0|x)$ from the original model as input and calculate the residual between the ideal and original predictive score to convert the original predictive score to ideal one during sales promotion. 

% \subsubsection{Architecture} We utilize a simple Multilayer Perceptron (MLP) to calculate the $w_{(x)}$ and $b_{(x)}$ in TransBlock module and the calculation depends on the hidden state $h_{(x)}$ of the penultimate layer of the CVR prediction model. The process is shown as follows, 
% \begin{equation}
% \begin{aligned}
% \label{eq:transblock} 
% \begin{bmatrix}
% w_{(x)} \\ b_{(x)} 
% \end{bmatrix} = W_\text{trans} \cdot h_{(x)}  + b_\text{trans} 
% \end{aligned} 
% \end{equation} 
% where $W_\text{trans}$ and $b_\text{trans}$ are trainable parameters. Note that in the optimization of fine-tuning, we treat the parameters of the original model and the parameters of TransBlock independently, i.e., we update the parameters of TransBlock with the large learning rate $\eta_{1}$ and optimize the parameters of the original model with a small learning rate $\eta_{2}$.

% \subsubsection{Inference} Since the output from TransBlock is the sum of the original model predictive score and residuals, we truncate it between (0,1) in order to ensure that the score has the probabilistic meaning, 
% \begin{equation}
% \begin{aligned}
% \label{eq:gating-unit}
% s = 
%     \left\{
%         \begin{matrix}
%             0, &  p_\text{trans}(y=1|x) < 0 \\
%             1, &  p_\text{trans}(y=1|x) > 1 \\
%             p_\text{trans}(y=1|x), &  \text{other}, \\
%         \end{matrix}
% \right. 
% \end{aligned} 
% \end{equation}
% where s is the calibrated predictive CVR in promotion. 


% \subsection{Industrial Deployment for Online Serving} 
% Here, we introduce our hands-on experience on practical deployment for the display advertising system in Alibaba. 

% First, we build a map-reduce task with day-level scheduling to parse the user behaviors from the traffic log, and construct the vector-based index as described in Section~\ref{sec:index_building}. When the index of the present day is finished, our system will calculate the similarity between the vector-based index of the present day and each historical day. Due to the acceptable amount of calculation, we only need to conduct the calculation of cosine distance by basic CPU operation. Finally,  the similarity results are stored in a SQL table which is updated on daily basis.

% Then, we conduct fine-tuning process on the real-time CVR prediction model. In practice, we use the real-time CVR prediction model as the classifier $f$, so we can obtain $p^h(\hat{y})$ from the real-time traffic log. Then, we utilize the real-time CVR prediction model to score the retrieved historical data to obtain the $q^h(x|y)$. Thereafter, we follow Eq.~\ref{eq:y} to work out $p^h{y}$, and then fine-tune the real-time CVR prediction model according to \chan{Eq. 3} to adopt the promotion. 

% Finally, the fine-tuned CVR prediction model is deployed online.



\section{The Proposed Method} 
\label{sec:model} 

\subsection{Observation} 
As mentioned before, recent CVR estimation methods, with or without delayed feedback modeling, are not able to predict CVR under such distribution saltation in sales promotions. To this end, we explore CVR estimation in sales promotions from a novel idea. 

First of all, through observing the trend of CVR, we find that the CVR between the sales promotions is closer than the promotions' and daily's. Thus, the intuitive idea is whether we could utilize the data of historical promotions to make the CVR model adapt to distribution during promotion. Thereafter, we analyze the statistics among the sales promotions and are aware of that the distribution of similar promotion approximately conform to the label shift assumption. 

\textbf{Assumption.} \textit{The distribution of similar promotion approximately conform to the label shift assumption. Specifically, we indicate the distribution of promotion A and B by $\mathcal{A}(x, y)$ and $\mathcal{B}(x,y)$, respectively, we can obtain $\mathcal{A}(x|y)=\mathcal{B}(x|y)$.} 
%Specifically, we indicate the distribution of promotion A and B by $\mathcal{A}(x, y)$ and $\mathcal{B}(x,y)$, respectively, we can obtain $\mathcal{A}(x|y)=\mathcal{B}(x|y)$. 

The intuitive understanding is that similar groups of users often select similar products in two similar promotions. To support this assumption, we counted the relevant data and verified its reasonable. \chan{TODO: data} 



Therefore, we propose a novel idea of CVR estimation: treating CVR estimation as a distribution adaptation problem under the \textit{label shift} assumption. Specifically, we propose the following two-stage algorithmic framework. Firstly, we design an efficient retrieval approach to search the historical data close to the current distribution in terms of day-level data. 
Secondly, we propose a distribution adaptation algorithm based on the importance-weighted Empirical Risk Minimization (ERM) framework, which can adapt the CVR model to the current target distribution based on the retrieved historical data and a fraction of real-time data without conversion label. Note that we find that the model perform overfitting while fine-tuning the model with historical data, that is the one-epoch phenomenon in recommendation system. Therefore, we designed a plug-and-play TransBlock module to alleviate the overfitting problem. 

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figs/vector_index_building.jpg} 
    \caption{The overall of the vector index building.} 
\end{figure*} 

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figs/p_x_given_y.jpg} 
    \caption{The overall of TransBlock.} 
\end{figure} 


%\subsection{Non-Parametric Vector-Based Retrieval} 
\subsection{Vector-Based Retrieval} 
%Firstly, we design an efficient retrieval approach to search the historical data close to the current distribution in terms of day-level data.
In the first step of the algorithm flow, we seek to obtain historical data that is similar with real-time distribution and approximately conform the label shift assumption. To industrial production deployment, we should avoid manual selection, and thus we build a vector-based retrieval approach in non-parametric manner to automatically retrieval similar data. In this following work, we set the retrieval granularity into day-level data, that is we shall select one day in historical data, whose data distribution is close to the current day's. 

\subsubsection{Vector-based index building} 
\label{sec:index_building}
Due to the lack of data for training, we do not follow the data-driven manner and return to classical non-parametric retrieval approach feature engineering. Specifically, we analyze observable data during the promotion and mined the feature factors that can represent to the characteristic of data distribution.  

First, we do not have access to the full target distribution, because our target is the current day-level data distribution $p(x,y)$, where $p(x)$ is available at the end of the day, and the waiting time for $p(y)$ is even as long as the attribution window. To this end, we explore the CVR trend during the promotion: the real-time conversion decreases significantly in the period before the discounted price takes effect, increases significantly when the discounted price takes effect, and decreases significantly again after the termination of the promotion. Therefore, we proposed to utilize the statistic from several preceding days to represent the unavailable current day. 
Meanwhile, we analyze the observable data. As shown in figure 2, we are aware that the trend of the display ratio of some specific categories is similar to the trend of CVR during the promotion. Therefore, we selected the display ratio of several representative categories as the feature factors for the retrieval. 

Specifically, we select seven representative product categories and count their display ratios in three preceding days of the current day. 
In the experiments, we find that if we consider statistics from the current day, it could significantly improve the performance of retrieval. Under the consideration of the retrieval effectiveness and the delay of the model serving, we also count the selected categories' display ratio of the first 10 hours of the current day. 
Thereafter, we build 28-dimensional vectors which are utilized as the retrieval indexes for the current day. 


\subsubsection{Retrieval approach} 
Based on the constructed vector-based index, we design a simple and efficient non-parametric vector retrieval methods. We calculate the cosine distance between the index of current day $\text{T}_\text{target}$ and the historical day $\text{T}_\text{history}$ as the similarity score: 
\begin{equation}
\begin{aligned} 
\label{eq:retieval} 
S_\text{similar} = \frac{V_\text{target} \cdot V_\text{history}}{|V_\text{target}| \cdot |V_\text{history}|} 
\end{aligned}
\end{equation}
Finally, we select the historical data with Top-3 similarity as the search result, so as to retrieve the most similar historical data. 

\subsection{CVR Estimation} 
After obtaining the available similar historical data through the above retrieval procedure, we conduct the estimation for accurate CVR with retrieved historical data and predictive score during the first 10 hours of the current day. Inspired by Black Box Shift Estimation (BBSE) approach for domain adaptation under label shift assumption, we regard the CVR estimation task as a domain adaptation task under label shift assumption, where the source domain is historical data. 

After obtaining the available similar historical data through the above retrieval procedure, we conduct the estimation for accurate CVR with retrieved historical data and predictive score during the first 10 hours of the current day. Inspired by Black Box Shift Estimation (BBSE) approach under label shift assumption, we design the CVR estimation under the importance-weighted ERM framework. The framework fine-tunes the current CVR prediction model on the following loss function, 
\begin{equation}
\begin{aligned}
\label{eq:retieval} 
%\mathcal{L} &= \frac{p(x,y)}{q(x,y)} \cdot \ell_{(x,y) \in q(x,y)}(x,y) \\ 
%&= \frac{p(x|y) \cdot p(y)}{q(x|y) \cdot q(y)} \cdot \ell_{(x,y) \in q(x,y)}(x,y) \\
%&= \frac{p(y)}{q(y)} \cdot \ell_{(x,y) \in q(x,y)}(x,y), 
\mathcal{L} &= \int \frac{p(x,y)}{q(x,y)} \cdot \ell(x,y) \ \mathrm{d} q(x,y) \\ 
&= \int \frac{p(x|y) \cdot p(y)}{q(x|y) \cdot q(y)} \cdot \ell(x,y) \ \mathrm{d} q(x,y) \\ 
&= \int \frac{p(y)}{q(y)} \cdot \ell(x,y) \ \mathrm{d} q(x,y) \\ 
\end{aligned}
\end{equation}
where $\ell$ is the loss function and it is cross-entropy in this work. $p(x,y)$ and $q(x,y)$ indicate the target distribution and historical distribution, respectively. As mentioned above, we assume the historical distribution and target distribution conform the \textit{label shift} setting, i.e., $p(x|y)=q(x|y)$. 

Since q(y) is known, we need to obtain the target label distribution p(y). However, it's hard to work out p(y), thus we change the target. As shown in Figure 1, the CVR ratio at any corresponding time between two days is relatively stable. We replace the $\frac{p(y)}{q(y)}$ by the ratio between the part of the day, as following, 
\begin{equation}
\begin{aligned}
\label{eq:retieval} 
\frac{p(y)}{q(y)} &\approx \frac{p^{h}(y)}{q^{h}(y)}, 
\end{aligned} 
\end{equation}
where $q^{h}(y)$ is also available, thereafter, we seek to solve the $p^h(y)$. 

Denote by $\hat{y} = f(x)$ the output of a fixed function $f$ which is a trained classifier, we arrive that $p^h(\hat{y}|y)=q^h(\hat{y}|y)$ when $p^h(x|y)=q^h(x|y)$ holds. %: $\mathcal{X} \rightarrow \mathcal{Y}$. 
Hereafter, we combine the law of total probability and arrive at
\begin{equation}
\begin{aligned}
\label{eq:s} 
p^h(\hat{y}) 
&= \int p^h(\hat{y}|y) \cdot p^h(y) \ \mathrm{d}y \\
&= \int q^h(\hat{y}|y) \cdot p^h(y) \ \mathrm{d}y, 
%&= \sum_{y \in (0,1)} p^h(\hat{y}|y) \cdot p^h(y) \\ 
%&= \sum_{y \in (0,1)} q^h(\hat{y}|y) \cdot p^h(y), 
\end{aligned} 
\end{equation} 
where we can obtain $p^h(\hat{y})$ and $q^h(\hat{y})$ through using classifier $f$ to score the $p^h(x)$ and $q^h(x)$. Due to the historical data being fully labeled, we can obtain $q^h(\hat{y}|y)$ from $q^h(\hat{y})$ according to the labels. For the convenience of representation, we write the above formula in matrix form as 

\begin{equation}
\begin{aligned}
\label{eq:matrix} 
D(\hat{y}) &= D(\hat{y}|y) \cdot D(y). 
\end{aligned} 
\end{equation} 
To solve $D(y)$, we can construct the following problem as 

\begin{equation}
\begin{aligned}
\label{eq:problem} 
\mathop{\arg\min}_{D(y)} \underbrace{|| D(\hat{y}|y) \cdot D(y) - D(\hat{y}) ||^2}_\text{(a)} + \underbrace{\lambda \cdot || D(\hat{y}) - D(y) ||^2 }_\text{(b)} 
\end{aligned} 
\end{equation} 
where Eq.(a) is to solve the Eq.~\ref{eq:matrix}, and Eq.(b) is a regularization constraint that constrains $\frac{p(y)}{q(y)}$ close to 1 for stability during training. \chan{cite} By solving Eq.~\ref{eq:problem}, we can obtain a closed-form solution $p^h(y)$ as
\begin{equation}
\begin{aligned}
\label{eq:y} 
D(y) = (D(\hat{y}|y)^TD(\hat{y}|y) + \lambda \mathbf{I})^{-1}(D(\hat{y}|y)^TD(\hat{y}) + \lambda D(y')). 
\end{aligned} 
\end{equation} 
Thus, we work out the $\frac{p^h(y)}{q^h(y)}$. Finally, we could fine-tune CVR prediction model according to \chan{Eq. 3} to adopt the promotion. 

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figs/transblock.jpg} 
    \caption{The overall of TransBlock.} 
\end{figure} 

\subsection{Tuning based on TransBlock Module} 
Due to the one-epoch phenomenon in recommender system, there will be terrible overfitting in fine-tuning procedure. Thus, we design a plug-and-play TransBlock module to assist fine-tuning and avoid the overfitting from historical data reusing. TransBlock is a stacking layer that is independent of the CVR model structure, and its goal is residuals of original predictive CVR score to ideal value.

\subsubsection{Motivation}  We use stacked design to protect the original predictive ability of the CVR model by optimizing the added stacking parameters more and original model less through historical data. Due to the sparsity of retrieved day-level historical data, we could only add a small amount of parameters to ensure convergence on the limited data. Thus, we design TransBlock as following intuitive considering, 
\begin{equation}
\begin{aligned}
\label{eq:transblock} 
p_\text{ideal}(y=1|x) = p(y=1|x) + \underbrace{v_{(x)} \cdot p(y=0|x)}_\text{(a)} - \underbrace{u_{(x)} \cdot p(y=1|x)}_\text{(b)}
\end{aligned} 
\end{equation} 
where the $p(y=1|x)$ and $p(y=0|x)$ are the conversion rate and non-conversion rate calculated by original CVR prediction model. The parts of above equation are 
\begin{itemize}%[leftmargin=*]
\item (a). \textit{Predicted probability of non-conversion but conversion, e.g., some products are rarely purchased on a daily basis, but are purchased frequently during sales promotion;} 
\item (b). \textit{Predicted probability of conversion but non-conversion, e.g., some products that are frequently purchased on a daily basis, but rarely during sales promotion,} 
\end{itemize} 
where $u_{(x)}$ and $v_{(x)}$ are the sample-related transfer probabilities. We further simplify the formula and arrive the calculation process of TransBlock, 
\begin{equation}
\begin{aligned}
\label{eq:transblock} 
p_\text{trans}(y=1|x) 
=& p(y=1|x) + v_{(x)} \cdot p(y=0|x) - u_{(x)} \cdot p(y=1|x) \\ 
=& p(y=1|x) + v_{(x)} \cdot p(y=0|x) - u_{(x)} \cdot (1-p(y=0|x)) \\
=& p(y=1|x) + (v_{(x)}+u_{(x)}) \cdot p(y=0|x) - u_{(x)} \\
\rightarrow & p(y=1|x) + \underbrace{w_{(x)} \cdot p(y=0|x) + b_{(x)}}_{w_{(x)}=v_{(x)}+u_{(x)}, b_{(x)}=-u_{(x)}}. 
%\small{\text{where} \ w_{(x)}=v_{(x)}+u_{(x)}, b_{(x)}=-u_{(x)}}
\end{aligned} 
\end{equation} 
As mentioned above, the TransBlock module takes the non-conversion probability $p(y=0|x)$ from the original model as input and calculate the residual between the ideal and original predictive score to convert the original predictive score to ideal one during sales promotion. 

\subsubsection{Architecture} We utilize a simple Multilayer Perceptron (MLP) to calculate the $w_{(x)}$ and $b_{(x)}$ in TransBlock module and the calculation depends on the hidden state $h_{(x)}$ of the penultimate layer of the CVR prediction model. The process is shown as follows, 
\begin{equation}
\begin{aligned}
\label{eq:transblock} 
\begin{bmatrix}
w_{(x)} \\ b_{(x)} 
\end{bmatrix} = W_\text{trans} \cdot h_{(x)}  + b_\text{trans} 
\end{aligned} 
\end{equation} 
where $W_\text{trans}$ and $b_\text{trans}$ are trainable parameters. Note that in the optimization of fine-tuning, we treat the parameters of the original model and the parameters of TransBlock independently, i.e., we update the parameters of TransBlock with the large learning rate $\eta_{1}$ and optimize the parameters of the original model with a small learning rate $\eta_{2}$.

\subsubsection{Inference} Since the output from TransBlock is the sum of the original model predictive score and residuals, we truncate it between (0,1) in order to ensure that the score has the probabilistic meaning, 
\begin{equation}
\begin{aligned}
\label{eq:gating-unit}
s = 
    \left\{
        \begin{matrix}
            0, &  p_\text{trans}(y=1|x) < 0 \\
            1, &  p_\text{trans}(y=1|x) > 1 \\
            p_\text{trans}(y=1|x), &  \text{other}, \\
        \end{matrix}
\right. 
\end{aligned} 
\end{equation}
where s is the calibrated predictive CVR in promotion. 


\subsection{Industrial Deployment for Online Serving} 
Here, we introduce our hands-on experience on practical deployment for the display advertising system in Alibaba. 

\chan{retieval} First, we build a map-reduce task with day-level scheduling to parse the user behaviors from the traffic log, and construct the vector-based index as described in Section~\ref{sec:index_building}. When the index of the present day is finished, our system will calculate the similarity between the vector-based index of the present day and each historical day. Due to the acceptable amount of calculation, we only need to conduct the calculation of cosine distance by basic CPU operation. Finally,  the similarity results are stored in a SQL table which is updated on daily basis.

\chan{real-world workflow} Then, we conduct fine-tuning process on the real-time CVR prediction model. In practice, we use the real-time CVR prediction model as the classifier $f$, so we can obtain $p^h(\hat{y})$ from the real-time traffic log. Then, we utilize the real-time CVR prediction model to score the retrieved historical data to obtain the $q^h(x|y)$. Thereafter, we follow Eq.~\ref{eq:y} to work out $p^h{y}$, and then fine-tune the real-time CVR prediction model according to \chan{Eq. 3} to adopt the promotion. 

Finally, the fine-tuned CVR prediction model is deployed online. 

\chan{real-world deployment: bank training path and fine-tune}

To adapt the novel workflow with historical data fine-tuning, we design a new dataset finetune workflow to the 

